On Joint Detection and Decoding in Short-Packet Communications

We consider a communication problem in which the receiver must first detect the presence of an information packet and, if detected, decode the message carried within it. We present general nonasymptotic upper and lower bounds on the maximum coding rate that depend on the blocklength, the probability of false alarm, the probability of misdetection, and the packet error probability. The bounds, which are expressed in terms of binary-hypothesis-testing performance metrics, generalize finite-blocklength bounds derived previously for the scenario when a genie informs the receiver whether a packet is present. The bounds apply to detection performed either jointly with decoding on the entire data packet, or separately on a dedicated preamble. The results presented in this paper can be used to determine the blocklength values at which the performance of a communication system is limited by its ability to perform packet detection satisfactorily, and to assess the difference in performance between preamble-based detection, and joint detection and decoding. Numerical results pertaining to the binary-input AWGN channel are provided.

==> Inputs/__latexindent_temp.tex <==
Author = {M. Khoshnevisan and J. N. Laneman},
	Journal = IEEE_J_IT,
	Month = jun,
	Number = {7},
	Pages = {5077-5094},
	Title = {Intermittent Communication},
	Volume = {63},
	Year = 2017}

==> Inputs/defs.tex <==
\usepackage{bm}
\usepackage{upgreek}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage{xspace}

\safemath{\mi}{I}
\safemath{\difent}{\mathrm{h}}		%differential entropy
\safemath{\NonnegReal}{\mathbb{R}^{+}}


\safemath{\indist}{\cdfP} %input distribution
\safemath{\outdist}{\cdfQ} %output distribution
\safemath{\inpdf}{\pdfp} %input pdf
\safemath{\outpdf}{\pdfq} %output pdf
\safemath{\testdist}{\cdfP} %the distribution of test P_{Z|W}

%\safemath{\tr}[#1]{\mathrm{tr}\left\lbrace #1  \right\rbrace}

\safemath{\powallocvec}{\vecv}
\safemath{\powalloc}{v}
\safemath{\encoder}{f} % the encoder of the code
\safemath{\decoder}{g} % the decoder of the code
\safemath{\msg}{J} % the message
\safemath{\csir}{\mathrm{r}}
\safemath{\csit}{\mathrm{t}}
\safemath{\csi}{\mathrm{csi}}
\safemath{\csirt}{\mathrm{rt}}
\safemath{\Rcsirt}{R_{\csirt}} %rate with CSIT
\safemath{\Rcsir}{R_{\csir}}
\safemath{\Rcsit}{R_{\csit}}
\safemath{\cohblock}{T}
\safemath{\blocklength}{n}
\safemath{\selbranches}{L}


\safemath{\Rnocsit}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rnocsi}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rgeneral}{R_{\mathrm{no,rt}}} %rate with general CSI condition
\safemath{\equalR}{R_{\mathrm{e}}}

\newcommand*\pFqskip{8mu}
\catcode`,\active
\newcommand*\pFq{\begingroup
        \catcode`\,\active
        \def ,{\mskip\pFqskip\relax}%
        \dopFq
}
\catcode`\,12
\def\dopFq#1#2#3#4#5{%
        {}_{#1}F_{#2}\biggl[\genfrac..{0pt}{}{#3}{#4};#5\biggr]%
        \endgroup
}

%------------------------------------
%		JOHAN
%------------------------------------
\safemath{\Rmax}{R^*(n,\epsilon)} %rate without CSIT
\safemath{\codewords}{K}
\safemath{\Rub}{\bar{R}(n,\epsilon)}
\safemath{\Rlb}{\underline{R}(n,\epsilon)}
\safemath{\rk}{\kappa}
\safemath{\rlos}{\bar{\matH}}
\safemath{\rnlos}{\tilde{\randmatH}}

\safemath{\randtemp}{K}

\safemath{\Vnocsit}{V_{\error}^{\mathrm{no}}}
\safemath{\Vcsit}{V_{\error}^{\mathrm{rt}}}

\safemath{\cadist}{F_C} %capacity distribution
\safemath{\cdistno}{F_{0}}
\safemath{\cdistcsit}{F_{1}}


\safemath{\deF}{d_0} %the derivative of F_C(\xi) %\left.\frac{d\cadist(\argpn)}{d\argpn}\right|_{\argpn=C_\error}

\safemath{\bl}{n} %block length
\safemath{\blt}{\tilde{\bl}}
\safemath{\error}{\epsilon} %prob of error
\safemath{\NumCode}{M}
\safemath{\RXant}{r}
%\safemath{\rxant}{r}
%\safemath{\txant}{t}
\safemath{\txantop}{t^{\ast}}
\safemath{\minant}{m}
\safemath{\minantop}{\minant^\ast}
\safemath{\snr}{\rho}
\safemath{\const}{k}
\safemath{\inset}{\setF} %the input power set
\safemath{\spanm}{\mathrm{span}}
\safemath{\ubb}{b_{0}}%upper bound of b_1,...,b_{r} of the matrix I+ H^H U H.

%%%%%%%%%%%MIMO%%%%%%%%%%%%%%%%%%%%
\safemath{\covmat}{\matU}
\safemath{\covmatY}{\matV}
\safemath{\randcmY}{\randmatV}

\safemath{\insetMIMO}{\setF_{\txant,\bl}}
\safemath{\insetcov}{\setU_{\txant}}
%\safemath{\condcov}{\matQ\succeq\mathbf{0},\tr(\matQ)\leq\snr}
\safemath{\condcov}{\matQ\in\insetcov}

\safemath{\BoundFU}{k_{\delta}}

\safemath{\argpn}{\xi} % the argument in the probability p(R)

\safemath{\angletest}{Z} %the angle test used in achievability part

\safemath{\Cnocsit}{C_{\epsilon}^{(0)}}
\safemath{\Ccsit}{C_{\epsilon}^{(1)}}

\safemath{\errorach}{P_\mathrm{e}} %the error in intuition part



\newcommand{\given}{\,\vert\,}				% conditioning
\newcommand{\ggiven}{\,\Vert\,}	
\safemath{\define}{\triangleq}			% definition
%\safemath{\fnorm}{\mathrm{F}}

\safemath{\altbl}{\tilde{\bl}}
\safemath{\constL}{k_{\mathrm{L}}}
\safemath{\constU}{k_{\mathrm{U}}}
\safemath{\funcL}{\tilde{q}}
\safemath{\funcU}{q}
\safemath{\ConstThm}{k_0}
%%%%%%%%%%%%%%%%used in the intuition part %%%%%%%%%%%%%
\safemath{\randrevec}{\randvecy}
\safemath{\revec}{\vecy}
\safemath{\trcwd}{\vecx}
\safemath{\randtrcwd}{\randvecx}
\safemath{\randnoisevec}{\randvecw}
\safemath{\transmitcwd}{\vecx_1} %the transmitted codeword in achievability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%used in the appendix of proving gamma=C_error + O(1/\bl) %%%%%%%%%%%%%
\safemath{\pickcwdnoch}{\vecx_0} %the chosen codeword x=[P,P,...,P]
\safemath{\pickcwd}{\vecx_0} %the chosen codeword x=[P,P,...,P]

\safemath{\inseqrand}{\randvecx}
\safemath{\inseq}{\vecx}

\safemath{\outseq}{\matY}
\safemath{\outseqrand}{\randmatY}

%used in the appendix of the proof of achievability
\safemath{\altT}{\widetilde{T}}
\safemath{\altU}{\widetilde{U}}
\safemath{\altmean}{\tilde{\mu}}
\safemath{\altvar}{\tilde{\sigma}}
\safemath{\altf}{\funcL}
\safemath{\altg}{\tilde{g}}
\safemath{\altgamma}{\tilde{\gamma}}
\safemath{\altdelta}{\tilde{\delta}}
\safemath{\altk}{\tilde{k}}
\safemath{\altconst}{\altk}
\safemath{\altbmLambda}{\widetilde{\bm{\Lambda}}}
\safemath{\constant}{\tilde{k}}

